Optical-Flow Wingbeat Counting in MuJoCo: A Comparison of Convolutional, Spiking, and Attention-Based Temporal Models

Visual monitoring of flapping-wing vehicles requires distinguishing individual wingbeats from motion strength and average frequency. This paper presents a controlled MuJoCo evaluation of wingbeat counting from signed optical flow observed by virtual cameras mounted on Crazyflie vehicles. Three flapping-wing models were recorded at optical distances of 1.5 and 3.0 m, producing 1,440 clips from 240 paired scene configurations with a scene-level 3:1 training-test split. A common spatial convolutional encoder was combined with a causal temporal convolutional network, a recurrent leaky integrate-and-fire spiking network, or causal self-attention. Each model predicted phase and activity, followed by the same directed-crossing event counter. The six existing convolutional models were retained, and all twelve new models were frozen before their test predictions were generated. Exact-count accuracies at 1.5 m were 96.67%, 95.00%, and 96.67%, respectively; at 3.0 m they were 94.44%, 92.22%, and 95.00%. All paired scene-bootstrap intervals for differences in exact-count accuracy included zero. Seven far-distance spiking-model clips had correct totals despite event-timing mismatches, demonstrating why total-count and event-level measurements must be reported together. The results support the feasibility of causal optical-flow counting in the tested setting and identify boundary-sensitive errors. They do not establish an architecture ranking across repeated training, real-flight robustness, or hardware efficiency.

==> tables/controls.tex <==
1.5 & CNN--TCN & 0/18 & 0/3 & 1 & 96.30 \\
1.5 & CNN--LIF & 0/18 & 0/3 & 0 & 94.44 \\
1.5 & CNN--Transformer & 0/18 & 0/3 & 0 & 96.30 \\
3.0 & CNN--TCN & 0/18 & 0/3 & 0 & 93.83 \\
3.0 & CNN--LIF & 0/18 & 0/3 & 1 & 91.36 \\
3.0 & CNN--Transformer & 0/18 & 0/3 & 1 & 94.44 \\


==> tables/diagnostics.tex <==
1.5 & CNN--TCN & 6/6 & 0/0 & 0 \\
1.5 & CNN--LIF & 8/8 & 1/1 & 0 \\
1.5 & CNN--Transformer & 6/6 & 0/0 & 0 \\
3.0 & CNN--TCN & 9/9 & 1/1 & 0 \\
3.0 & CNN--LIF & 10/17 & 4/11 & 7 \\
3.0 & CNN--Transformer & 7/7 & 2/2 & 0 \\


==> tables/events.tex <==
1.5 & CNN--TCN & 1964 & 1958 & 1958 & 0 & 6 & 100.000 & 99.695 \\
1.5 & CNN--LIF & 1964 & 1957 & 1956 & 1 & 8 & 99.949 & 99.593 \\
1.5 & CNN--Transformer & 1964 & 1958 & 1958 & 0 & 6 & 100.000 & 99.695 \\
3.0 & CNN--TCN & 1964 & 1956 & 1955 & 1 & 9 & 99.949 & 99.542 \\
3.0 & CNN--LIF & 1964 & 1958 & 1947 & 11 & 17 & 99.438 & 99.134 \\
3.0 & CNN--Transformer & 1964 & 1959 & 1957 & 2 & 7 & 99.898 & 99.644 \\


==> tables/overall.tex <==
1.5 & CNN--TCN & 174/180 & 96.67 & [93.89, 98.89] & 0.0333 & 0.998470 \\
1.5 & CNN--LIF & 171/180 & 95.00 & [91.67, 97.78] & 0.0500 & 0.997705 \\
1.5 & CNN--Transformer & 174/180 & 96.67 & [93.89, 98.89] & 0.0333 & 0.998470 \\
3.0 & CNN--TCN & 170/180 & 94.44 & [91.11, 97.22] & 0.0556 & 0.997449 \\
3.0 & CNN--LIF & 166/180 & 92.22 & [87.78, 96.11] & 0.0778 & 0.992861 \\
3.0 & CNN--Transformer & 171/180 & 95.00 & [91.67, 97.78] & 0.0500 & 0.997706 \\


==> tables/paired.tex <==
1.5 & CNN--LIF $-$ CNN--TCN & -1.67 [-4.44, +1.11] & -0.000766 [-0.002098, +0.000521] \\
1.5 & CNN--Transformer $-$ CNN--TCN & +0.00 [-1.67, +1.67] & +0.000000 [-0.000755, +0.000753] \\
1.5 & CNN--Transformer $-$ CNN--LIF & +1.67 [-0.56, +4.44] & +0.000766 [-0.000264, +0.001938] \\
3.0 & CNN--LIF $-$ CNN--TCN & -2.22 [-6.67, +1.67] & -0.004588 [-0.008936, -0.001059] \\
3.0 & CNN--Transformer $-$ CNN--TCN & +0.56 [-1.67, +2.78] & +0.000257 [-0.000810, +0.001371] \\
3.0 & CNN--Transformer $-$ CNN--LIF & +2.78 [-1.11, +7.22] & +0.004845 [+0.001285, +0.009106] \\


==> tables/per_target.tex <==
1.5 & CNN--TCN & RLFlapping & 58/60 & 96.67 & 0.033 & 0.99840 \\
1.5 & CNN--TCN & flappy\_v2 & 60/60 & 100.00 & 0.000 & 1.00000 \\
1.5 & CNN--TCN & BIRD\_SIM & 56/60 & 93.33 & 0.067 & 0.99707 \\
1.5 & CNN--LIF & RLFlapping & 56/60 & 93.33 & 0.067 & 0.99680 \\
1.5 & CNN--LIF & flappy\_v2 & 58/60 & 96.67 & 0.033 & 0.99847 \\
1.5 & CNN--LIF & BIRD\_SIM & 57/60 & 95.00 & 0.050 & 0.99780 \\
1.5 & CNN--Transformer & RLFlapping & 57/60 & 95.00 & 0.050 & 0.99760 \\
1.5 & CNN--Transformer & flappy\_v2 & 60/60 & 100.00 & 0.000 & 1.00000 \\
1.5 & CNN--Transformer & BIRD\_SIM & 57/60 & 95.00 & 0.050 & 0.99780 \\
3.0 & CNN--TCN & RLFlapping & 57/60 & 95.00 & 0.050 & 0.99760 \\
3.0 & CNN--TCN & flappy\_v2 & 58/60 & 96.67 & 0.033 & 0.99847 \\
3.0 & CNN--TCN & BIRD\_SIM & 55/60 & 91.67 & 0.083 & 0.99633 \\
3.0 & CNN--LIF & RLFlapping & 57/60 & 95.00 & 0.050 & 0.99760 \\
3.0 & CNN--LIF & flappy\_v2 & 54/60 & 90.00 & 0.100 & 0.98471 \\
3.0 & CNN--LIF & BIRD\_SIM & 55/60 & 91.67 & 0.083 & 0.99633 \\
3.0 & CNN--Transformer & RLFlapping & 57/60 & 95.00 & 0.050 & 0.99760 \\
3.0 & CNN--Transformer & flappy\_v2 & 57/60 & 95.00 & 0.050 & 0.99770 \\
3.0 & CNN--Transformer & BIRD\_SIM & 57/60 & 95.00 & 0.050 & 0.99780 \\

